Vulnerability of Text-to-Image Models to Prompt Template Stealing: A Differential Evolution Approach

Prompt trading has emerged as a significant intellectual property concern in recent years, where vendors entice users by showcasing sample images before selling prompt templates that can generate similar images. This work investigates a critical security vulnerability: attackers can steal prompt templates using only a limited number of sample images. To investigate this threat, we introduce Prism, a prompt-stealing benchmark consisting of 50 templates and 450 images, organized into Easy and Hard difficulty levels. To identify the vulnerabity of VLMs to prompt stealing, we propose EvoStealer, a novel template stealing method that operates without model fine-tuning by leveraging differential evolution algorithms. The system first initializes population sets using multimodal large language models (MLLMs) based on predefined patterns, then iteratively generates enhanced offspring through MLLMs. During evolution, EvoStealer identifies common features across offspring to derive generalized templates. Our comprehensive evaluation conducted across open-source (INTERNVL2-26B) and closed-source models (GPT-4o and GPT-4o-mini) demonstrates that EvoStealer's stolen templates can reproduce images highly similar to originals and effectively generalize to other subjects, significantly outperforming baseline methods with an average improvement of over 10%. Moreover, our cost analysis reveals that EvoStealer achieves template stealing with negligible computational expenses. Our code and dataset are available at https://github.com/whitepagewu/evostealer.

==> tables/cost.tex <==

\begin{table}[!t]
    \centering
    \renewcommand{\arraystretch}{0.9}  % Increasing the row height for better readability

    \begin{tabular}{cccc}
        \toprule
         & \textbf{API } & \textbf{Token} & \textbf{Image}\\
        \midrule
        Volume  & 144 & 119.1k & 34 \\ 
         Cost & - &- & - \\
        \bottomrule
    \end{tabular}
    \caption{}
    \label{tb:cost}
\end{table}


==> tables/models.tex <==
\begin{table}[ht]
    \centering
    \setlength\tabcolsep{6pt} % Adjust the space between table columns
    \renewcommand{\arraystretch}{1}% Adjust the height of table rows
    \scalebox{0.9}{ % Adjust the scale of the table
    \begin{tabular}{ccccc}
        \toprule
        \textbf{Model} & \textbf{DINO } & \( \textbf{CLIP}_{\textit{img}} \) & \( \textbf{CLIP}_{\textit{txt}} \) & \textbf{Avg.}\\
        \midrule
        \multicolumn{5}{c}{\textbf{In-Domain}} \\ 
        \midrule\midrule
        InternVL2-26B & 72.32 & 82.71 & 67.31 & 74.11\\
        GPT-4o-mini  & 72.17 & 82.52 & 70.41 & 75.03\\
        GPT-4o  & 72.54 & 83.32 & 72.55 & 76.14\\
        \midrule
        \multicolumn{5}{c}{\textbf{Out-of-Domain}} \\ 
        \midrule\midrule
        InternVL2-26B & 70.29 & 81.34 & 66.59 & 72.74\\
        GPT-4o-mini  & 70.33 & 82.19 & 69.92 & 74.15\\
        GPT-4o  & 71.07 & 82.21 & 71.78 & 75.02\\

        \bottomrule
    \end{tabular}}
    \caption{Comparison of performance between InterVL2-26B, GPT-4o-mini, and GPT-4o.}
    \label{tb:models}
\end{table}



